Privacy-Engineered Value Decomposition Networks for Cooperative Multi-Agent Reinforcement Learning

In cooperative multi-agent reinforcement learning (Co-MARL), a team of agents must jointly optimize the team's long-term rewards to learn a designated task. Optimizing rewards as a team often requires inter-agent communication and data sharing, leading to potential privacy implications. We assume privacy considerations prohibit the agents from sharing their environment interaction data. Accordingly, we propose Privacy-Engineered Value Decomposition Networks (PE-VDN), a Co-MARL algorithm that models multi-agent coordination while provably safeguarding the confidentiality of the agents' environment interaction data. We integrate three privacy-engineering techniques to redesign the data flows of the VDN algorithm, an existing Co-MARL algorithm that consolidates the agents' environment interaction data to train a central controller that models multi-agent coordination, and develop PE-VDN. In the first technique, we design a distributed computation scheme that eliminates Vanilla VDN's dependency on sharing environment interaction data. Then, we utilize a privacy-preserving multi-party computation protocol to guarantee that the data flows of the distributed computation scheme do not pose new privacy risks. Finally, we enforce differential privacy to preempt inference threats against the agents' training data, past environment interactions, when they take actions based on their neural network predictions. We implement PE-VDN in StarCraft Multi-Agent Competition (SMAC) and show that it achieves 80% of Vanilla VDN's win rate while maintaining differential privacy levels that provide meaningful privacy guarantees. The results demonstrate that PE-VDN can safeguard the confidentiality of agents' environment interaction data without sacrificing multi-agent coordination.

==> privacy_policy.tex <==
\subsection{PRIVACY POLICY}
According to the Contextual Integrity Theorem \cite{}, privacy is a socially created need and a contextual concept. In particular, the theorem explains that \textit{inappropriate information flows} lead to privacy concerns in society. What constitutes inappropriate information flows depends on five parameters in the theorem's view: the subject of the information flow, its senders and recipients, information types, and transmission principles such as consent. Beyond privacy concerns, the theorem contends that the interests of the affected parties, ethical and political values in society, and contextual functions, purposes, and values ultimately determine the ethical legitimacy of information flows. 

Based on Contextual Integrity, algorithms cannot have innate privacy issues because they can be deployed in various contexts and may or may not establish inappropriate information flows. As a result, we approach privacy for Co-MARL algorithms withn a scenario-based privacy analysis methodology in which we assume certain privacy concerns and develop algorithmic solutions that preempt them. 

We assume that the agents' environment interaction data in Co-MARL contain privacy-sensitive information such that any information flow that carries this information type is inappropriate. The assumption implies that the existence of an upstream unit such as a central optimizer that consolidates replay buffers in centralized training algorithms violates privacy. Moreover, any information flow that does not necessarily carry environment interaction data but exposes it to indirect inference reasoning violates privacy. For example, transmitting the output of deterministic functions of environment interaction data, such as action-value functions, violates privacy as well.   

Our privacy analysis methodology begins with a ``technical privacy policy''. This policy is not the same as those displayed on websites, but similar to R. Anderson's security policy for security engineering \cite{anderson2020security}, it is rather a short and verifiable statement of the specifications that our privacy assumptions imply for Co-MARL. The technical privacy policy that we consider is as follows:
\begin{itemize}
    \item Sharing environment interaction data in the clear is forbidden with any other entity.
    \item Otherwise, the agents may engage in data sharing if such data sharing leads to higher team rewards and there exist mathematical guarantees that ensure the confidentiality of the sender agent's environment interaction data and that of other agents.
\end{itemize}
